Music Composition Using Quantum Annealing

With the emergence of quantum computers, a new field of algorithmic music composition has been initiated. The vast majority of previous work focuses on music generation using gate-based quantum computers. An alternative model of computation is adiabatic quantum computing (AQC), and a heuristic algorithm known as quantum annealing running in the framework of AQC is a promising method for solving optimization problems. In this chapter, we lay the groundwork of music composition using quantum annealing. We approach the process of music composition as an optimization problem. We describe the fundamental methodologies needed for generating different aspects of music including melody, rhythm, and harmony. The discussed techniques are illustrated through examples to ease the understanding. The music pieces generated using D-Wave quantum annealers are among the first examples of their kind and presented within the scope of the chapter. The text is an unedited pre-publication version of a chapter which will appear in the book "Quantum Computer Music", Miranda, E. R. (Editor).

==> markov_random_fields.tex <==
\subsection{Markov Random Fields}
Now, we will explore another tool that can be used to model our problems when using quantum annealing.
\subsubsection{Markov Chains}\label{sec: markovchains}

Suppose that we want to predict the weather of the following day. Is it more likely that tomorrow will be cold? Or perhaps, will it be rainy? To solve the problem, we could make the following analysis: let's say that the probability of a cold day in our city is 1/4; if today it is cold, the likelihood of tomorrow being cold would be the joint probability of these events, that is, $P(\text{today is cold and tomorrow is cold}) = \frac{1}{4} \cdot \frac{1}{4} = \frac{1}{16}
$. This probability seems too low, and usually, cold days follow one another in a row. If today is the first cold day in a while, a probability of 1/16 for tomorrow being also a cold day does not reflect our experience entirely.

Markov's revolutionary idea was to approach this problem in a different way; instead of viewing each probability as independent from one day to another, he decided to consider the present state as a necessary piece of information, the only one actually, for calculating the weather of the next day. In our analogy, this is like saying that the probability of being cold tomorrow depends only on the state of today's weather. If today it is cold, the probability of tomorrow being cold should be higher than it would be if today is too hot instead. With this approach, a sequence of weather states can give rise to a chain of events that satisfies what it is called the \textit{Markovian property}.


Consider a discrete-time stochastic process, this is, a sequence of random variables $\{X_{n\geq0}\}$, with state space $E$. Here, we will consider a countable state space. If for all integers $n\geq 0$ all the states $i_0, i_1, ..., i_{n-1}, i, j$ satisfy 
\begin{equation} \label{eq:mc}
P(X_{n+1}=j\vert X_n=i, X_{n-1}= i_{n-1}, \dots, X_0=i_0)= P(X_{n+1}=j\vert X_n=i),
\end{equation}
we say that the process is a \textit{Markov chain}.

In our example, the state space has three states, namely $\{\text{hot, cold, rainy}\}$. As for the conditional probabilities $ P_{i,j}\equiv P(X_{n+1}=j\vert X_n=i)$ (the probability of $j$ happening tomorrow given that $i$ occurs today), it is customary to arrange them in a matrix called the \textit{transition matrix} as depicted in Table \ref{table: markov}.  For instance, $P_{\text{hot,cold}} = 1/4$ represents the probability of a cold day happening tomorrow, given that a hot day occurs today.

\begin{table}[h!]
	\centering
	\begin{tabular}{ |c|ccc| } 
		\hline
		& hot & cold & rainy \\
		\hline
		hot  & 1/2 & 1/4 & 1/4 \\ 
		cold & 1/6 & 1/2 & 1/3 \\ 
		rainy  & 1/8 & 3/8 & 1/2 \\ 
		\hline
	\end{tabular}
	\caption{Transition probabilities for the Markov chain with the state space $\{$hot, cold, rainy$\}$.}
	\label{table: markov}
\end{table}

A transition matrix can also be visualized as a graph whose vertices represent the states of $E$. This graph has an oriented edge from $i$ to $j$ that will appear labeled with the probability $P_{i,j}$. The graph representation for our example is given in Fig. \ref{fig:markov}. 

\begin{figure}[h!]
	\begin{center}
		\includegraphics[scale=0.2]{graph}
		\caption{The graph representation for the Markov chain with state space hot, cold, rainy. Each transition is labeled with the appropriate probability.}
		\label{fig:markov}
	\end{center}
\end{figure}

\subsubsection{Markov Random Fields}
Let's generalize the concept of a Markov chain and introduce the Markov Random Field. A \textit{Markov Random Field} (MRF) or \textit{Markov Network} is a set of random variables that form an undirected graph which obeys the Markovian property \cite{spitzer1971markov, preston1973generalized}. Random variables are represented by the nodes of the network (the vertices of the graph). Each random variable can take values from a finite set, and an assignment to the variables is called a \textit{configuration}. Any pair of random variables that are not connected are conditionally independent. 

In the example visualized in Fig. \ref{fig:mrf}, we can observe several fully connected subgraphs of the graph. We denote these subgraphs as \textit{cliques}. A \textit{potential} function is defined over the cliques of the graph, assigning a value to every configuration of the clique. It is important to note though that, these values need not represent actual probabilities, that is, they may not add up to 1.

\begin{figure}[h!]
	\begin{center}
		\includegraphics[scale=0.27]{field}
		\caption{An example of a Markov Random Field.}
		\label{fig:mrf}
	\end{center}
\end{figure}

Concerning the potential functions, these are associated with an energy function. The total energy is defined as the sum over all clique potentials. High energy will indicate a low probability for a certain configuration to happen, and conversely, low energy will suggest that a specific configuration has more chances to occur. Although we do not go into the details of the energy calculation here, we refer interested readers to \cite{Kindermann1980MarkovRF}.

From Fig.~\ref{fig:mrf}, let's choose the clique $C_{0}=\{C,E\}$ with $C\in\{0,1\}$ and $E\in\{0,1\}$, that is $C$ and $E$ are binary random variables. We can define the potentials for the different configurations of the clique as shown in Table \ref{table:potentials}.

\begin{table}[h!]
	\centering
	\begin{tabular}{ |c|c|c| } 
		\hline
		$C$ & $E$ & $p(C,E)$ \\
		\hline
		0 & 0 & 0.3 \\ 
		\hline
		0 & 1 & 0.9 \\
		\hline
		1 & 0 & 2.6 \\
		\hline
		1 & 1 & 5.0 \\
		\hline
	\end{tabular}
	\caption{Potentials for the clique $C_{0}=\{C,E\}$ from Fig. \ref{fig:mrf}. }
	\label{table:potentials}
\end{table}


We will be primarily interested in the configuration with the highest probability of occurrence, equivalently the lowest energy. This is where the idea of \textit{optimization} comes into play. The idea here is to encode the states of interest as the nodes of the network and then define the potentials so that using an optimization algorithm the lowest energy configuration is obtained. Markov random fields have been extremely popular for vision and image processing \cite{blake2011markov}.




\subsubsection{Quantum Annealing and Markov Random Fields}

Markov Random Fields are inspired by the Ising Model \cite{Kindermann1980MarkovRF} and can be viewed as an attempt for generalization of the 2-local Ising Model traditionally defined over a lattice. From the view of probability theory, the probability that each particle ends up in state -1 or 1 depends only on the spin values of its neighbors, hence satisfying the Markovian property. Therefore, the Ising model is indeed a special case of MRF, where there are cliques of sizes 1 and 2 only, and the state space is $\{-1,1\}$. 


As mentioned previously in this chapter, quantum annealing provides a way to take advantage of the properties of a quantum system to find solutions for optimization problems. Through the use of tools such as the Ocean software development kit provided by D-Wave, one can create a Markov network and use D-Wave machines to sample configurations of the random variables with the lowest energy. This is accomplished by D-Wave, by creating a QUBO model from the potentials of the Markov network as described below.

Given random variables $X_1$ and $X_2$ with potentials $\phi_{00},\phi_{01},\phi_{10},\phi_{00}$ where $\phi_{ij}$ is the potential for $X_1=i$ and $X_2=j$, the corresponding QUBO formulation is defined as 
\begin{equation}\label{eq:qubomrf}
(\phi_{10} - \phi_{00}) x_1 + (\phi_{10} - \phi_{00}) x_2 + (\phi_{11} - \phi_{10} - \phi_{01} + \phi_{00}) x_1x_2 + \phi_{00}.
\end{equation}



